A Survey of Deep Network Solutions for Learning Control in Robotics: From Reinforcement to Imitation

Deep learning techniques have been widely applied, achieving state-of-the-art results in various fields of study. This survey focuses on deep learning solutions that target learning control policies for robotics applications. We carry out our discussions on the two main paradigms for learning control with deep networks: deep reinforcement learning and imitation learning. For deep reinforcement learning (DRL), we begin from traditional reinforcement learning algorithms, showing how they are extended to the deep context and effective mechanisms that could be added on top of the DRL algorithms. We then introduce representative works that utilize DRL to solve navigation and manipulation tasks in robotics. We continue our discussion on methods addressing the challenge of the reality gap for transferring DRL policies trained in simulation to real-world scenarios, and summarize robotics simulation platforms for conducting DRL research. For imitation leaning, we go through its three main categories, behavior cloning, inverse reinforcement learning and generative adversarial imitation learning, by introducing their formulations and their corresponding robotics applications. Finally, we discuss the open challenges and research frontiers.

==> secs/introduction-bk.tex <==
\section{Introduction}
%introduction of robotics trend and problem
\IEEEPARstart{R}{obots} have been more often in use for both industry and daily
life along the rapid advancement in science and technology over the last
decades. It is convinced that robotics will be
indispensable in the future: warehousing robots, autopilot cars,
unmanned aerial vehicles, industrial robots, \textit{etc}. Everyone
from this era has direct experience of this inevitable trend.
However, there are still some unsolved challenges, among which \hl{perception and sensory-motor} are taking important positions.
Deep-learning (\textit{DL}) is the leading breakthrough technique to overcome these challenges.
%A key representative of the advancement in
%deep-learning is the application of the GO game.
%A deep-learning enhanced agent \citep{silver2016mastering} beat the best human player in this game which was once to be considered as the most difficult problem for artificial intelligence
%\citep{bengio2009learning}.
In this paper, we try to survey the
deep-learning related research for solving robotic related
\hl{sensory-motor} problems with emphasis to mobile robotic challenges.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{figs/supervisenetwork}
    % \caption{A typical \textit{CNN} framework for robotics. Raw sensor information (depth image from an RGB-D sensor) was taken as input to connect with the robot control command directly \citep{tai2016deep}.}
    \caption{A typical \textit{CNN} framework for robotics.
    Raw sensor information (e.g. depth image from an RGB-D sensor) is fed directly into a deep network,
    which then outputs the control command.} %\citep{tai2016deep}.}
    \label{fig:coordinatefigure}
\end{figure}

%problem to be solved
% We divide \textit{DL} methods for robotic problems into two categories:
% perception and control systems. Firstly, the perception of the environment
% relies on various sensor information. Classical methods
% extract information from the raw sensor readings based on
% artificially designed complex features (\textit{e.g.},
% \textit{SIFT}
% \citep{lowe1999object,lowe2004distinctive,liu2014topological},
% \textit{SURF} \citep{bay2006surf,bay2008speeded}, \textit{ORB}
% \citep{rublee2011orb,moreno2015constant,mur2015orb}). Most of the
% classical methods are constrained by the adaptivity to generic
% environments. Regarding unstructured dynamic environments,
% such as hybrid environments for autonomous cars or complicated
% production lines for industrial robots, those
% methods are prone to errors.
%In addition, most of these traditional methods cannot run in real time.
The process from sensory information to motion is generally
regarded as a sensory-motor control system.
A wider scope of such systems includes mobile navigation, planning,
grasping and assistant system, etc. Based on environmental perception,
appropriate decision-making policy or control strategy should be
realized effectively and efficiently. For example, the navigation
for mobile robots with rational motion and coarse precision is considered as solved
\citep{cadena2016past}. However, in challenging environments or with high expectation on the precision over large-scale,
further research for robust methods are still needed. We show
some \textit{DL}-based solutions for this problem.

% why deep-learning can do that
Deep-learning has been widely used to solve artificial intelligent
problems \citep{bengio2009learning}. With benefits from the
improvement of computational hardware, multiple processing layers,
like deep convolution neural network, reached great success in solving
complicated estimation problems. The multiple levels of abstraction also
indicates the great advantage in high-dimensional data representation and
processing
\citep{lecun2015deep} compared with other state-of-the-art methods.
Convolutional Neural Networks (\textit{CNN}) have won almost all of
contests in machine learning and pattern recognition, for example
image recognition \citep{he2015deep}, object detection
\citep{ren2015faster}, semantics segmentation \citep{chen2016deeplab},
audio recognition \citep{deng2013new}, and natural language processing
\citep{cambria2014jumping}. Deep-learning is capable of extracting
multi-level features from raw sensor information directly without any
handcrafted designs. It implies the great potential of deep-learning
in future applications. Novel deep-learning frameworks
(\textit{e.g.,} \textit{Caffe} \citep{jia2014caffe},
\textit{Tesnforflow} \citep{abadi2016tensorflow}) and algorithms have
been created constantly, which has also accelerated this progress
\citep{lecun2015deep}.

\begin{figure}[t]
    \includegraphics[width=1\linewidth]{figs/countnum}
    \caption{\textit{Deep-learning Robot} keywords related paper count and citation count in the last decade until Jan 2018. A drastically increasing trend of both the count of \textit{Deep-learning Robot} related publications and citations can be easily observed.}
    % It is obvious that both the count of \textit{Deep-learning Robot} related publications and citations have been increasing dramatically.}
    \label{fig:dlr}
\end{figure}
% reference 157 189 159 160 88 82 70 46 51 49
%12 29 16 27 20 8 9 14 14 8 (2016 2007)
% paper number 20 40 16 9 6 3 4 3 5 7

Since the potential of \textit{DL},
%has been released and revealed,
%As an appropriate solution for bottlenecks in robotics perception and
%control,
more researchers have progressively explored other possibilities and
applications using deep-learning related methods, especially in robotics.
Figure \ref{fig:dlr} depicts the increasing trend of
\textit{Deep-learning Robot} related publications over the past decades.
We believe the trend will keep on exploding for the near future.

\subsection{Scope and paradigms}
\label{sec:paradigm}

We give a broad survey of the current development of \textit{DL} in
robotics and discuss its open challenges for mobile robotics in sensory-motor policies.
Since both robotics and deep-learning as themselves contain a large number of aspects and wide paradigms.
We would like to constraint our scope within the following paradigms.

\begin{itemize}
\item \textit{Robot:} This paper mainly talks about mobile robots, unmanned aerial vehicle, manipulators, \textit{etc}.
Other forms such as nano-robots, emotional robots, humanoid or designation are not included.
%\item \textit{Perception:} The raw sensor inputs are constrained within cameras, depth cameras, Lidar, \textit{etc}. The perception here refers to those as auxiliary for mobile robotic tasks. e.g. speech recognition is also essential for the robot and human interaction, but since it is irrelevant to robotic research thus not included in this survey.
\item \textit{Sensory-motor:} \hl{We consider the transformation from sensory
input to control output as a sensory-motor control system. We show a
lot of robotic sensory-motor problems aided by \textit{DL}, including
mobile robots navigation, robot arms grasping, path planning,
\textit{etc}, through the direct or indirect connection between the
sensory information and the control command. We also survey the
deep-learning related Model-Predictive Control research, where the
dynamics transition model is learned from deep neural networks.
Other control theory-related paradigms such as system stability, controllability and observability are not included.}
\item \textit{Deep-learning:} Deep hierarchical model and its
extensions or enhancement by other learning methods are all considered as
deep-learning models in this survey,
such that we try to maximize the scope of related methods while focusing on the applications to mobile robots.
\end{itemize}

Deep-learning provides hands-on and practical solutions to various fields with aid from data.
Note that a minority that is beyond but highly related to robotics is also discussed.
We believe the cross-fertilization among these fields is inspiring to the readers.

The paper starts with presenting a brief introduction to deep-learning
both from the machine learning point-of-view and robotics in Section
\ref{sec:dlml} and Section \ref{sec:dlro}. A large variety of tasks
where deep-learning has been successfully applied to mobile robotics is
presented in this paper.
%Section \ref{sec:percetpion} surveys the
%application of deep-learning in robotics perception. The perception of
%robotics is divided into two aspects: the object detection problem;
%the environment and place recognition problem.
%Section \ref{sec:control} deals with deep-learning in \hl{robotics sensory-motor system}.
Recent improvements in Deep Reinforcement Learning (\textit{DRL})
and Deep Inverse Reinforcement Learning (\textit{DIRL}) are
highlighted. Future directions are presented at the end of these
sections, followed by conclusions in Section \ref{sec:conclu}.


% \textit{DL} is a typical machine learning method. Machine learning is
% typically classified into three categories: supervised learning,
% unsupervised learning, and reinforcement learning
% \citep{russell2003artificial,bishop2006pattern}.
%
% \textbf{Supervised Learning} The most common form of machine learning is supervised learning. In supervised learning, an objective function is computed to measure the error between the output and the desired labeled with a cost function. The final output is the one with the minimum cost.
%
% \textbf{Unsupervised Learning} Compared with supervised learning, there is no labeled data provided in unsupervised learning. It aims to find the hidden pattern, structure or features embedded with the data. The primary form of learning for humans and animals is unsupervised learning, i.e. to explore the world not from being told so but from observation.
%
% \textbf{Reinforcement Learning} In reinforcement learning, an agent is defined to explore and exploit the space of possible strategies. Feedback in form of reward or cost from the dynamic environment is referred as the outcome of the chosen action.
%
% All above are inherently tackling features from the training data.
% Supervised and unsupervised learning intend to locate the nearest
% neighbors in feature spaces through supervision, and reinforcement
% learning is a stochastic search problem to identify the highest-reward
% policy by trial-and-error. Internal adjustable parameters of these models are
% called weights. For supervised learning and reinforcement learning,
% weights of the models are motivated to converge by gradient descent
% methods. Traditionally, machine learning methods are seriously limited
% to the feature quality and complexity. For example,
% \citet{lecun2015deep} described a selectivity-invariance dilemma for supervised learning:
% representations abstracted by extractors should be both selective for
% discrimination and invariant to irrelevant aspects. Generic non-linear
% features like kernel methods \citep{smola1998learning} can boost the
% performance of the classifiers, but such kind of features always brings
% over-fitting problems for the training samples. Hand-crafted feature
% extractor is another useful method conventionally, but complicated
% domain expertise is essential for such kind of extractors.
% Deep-learning aims to provide a general-purpose learning procedure so
% that high-quality features can be learned autonomously and
% efficiently from data.

%deep-learning
\textit{DL} structure always involves a multilayer stack of learning
and non-linear modules (layers) \citep{lecun2015deep}, which increase
both the selectivity and the invariance. We also consider this is the
primary contribution and the advantage of deep-learning.
Feature representations in unsupervised learning and reinforcement
learning also benefit from that.

\begin{figure}[!ht]
     \centering
     \includegraphics[width=1\linewidth]{figs/RNN.pdf}
     % \caption{Recurrent Neural Network Structure. The left is the typical \textit{RNN} structure. The right part is the unfolding version where the previous information is transformed to the later time step.}
     \caption{Recurrent Neural Network Structure. Left: the typical \textit{RNN} structure.
     Right: the unfolded version to transform the previous information to later time steps.}
     \label{fig:rnn}
\end{figure}

The complexity of modules in \textit{DL} model are dramatically
increasing in the last several years to be sensitive to minute details
so that the abstracted representations are more meaningful and precise
for specific targets \citep{krizhevsky2012imagenet,simonyan2014very}.
A state-of-the-art image classification method can use a structure with
more than 150 layers \citep{he2015deep}. The realization of such a huge
multilayer structure benefits from the hardware development like
Graphics Processing Unit (\textit{GPU}). The enormous calculation
ability accelerated by high-performance hardware architecture make it
possible to construct the huge deep-learning modules combination.
Normally, purely accumulating the deep-learning modules may not lead
the weights of the model to converge. Several reasonable training
strategies like \textit{batch-normalization} \citep{ioffe2015batch}
and \textit{drop-out} \citep{srivastava2014dropout} also make a
contribution to the deep-learning development.

Typical deep-learning modules include pure Deep Neural Networks
(\textit{DNN}), Convolutional Neural Networks (\textit{CNN})
\citep{le1990handwritten}, and their transformations like Recurrent
Neural Networks (\textit{RNN}) \citep{pineda1987generalization},
Long-Short Term Memory (\textit{LSTM}) \citep{hochreiter1997long},
\textit{etc}. As shown in Figure \ref{fig:coordinatefigure},
\textit{CNN} is a combination of convolutional processing with learned
filters. Normally a \textit{CNN} model also consisted of pooling
layers for dimension reduction and activation layers for the non-linearity increasing.

Except for instant input, the output of \textit{RNN} is also
influenced by the prior information. Like \textit{CNN} share
features through space, \textit{RNN} can be regarded as a feature
sharing structure along time.
%As shown in the left of Figure
%\ref{fig:rnn}, there is a loop in the inner net of \textit{RNN} so
%that information of last time step is allowed to be kept in the
%neuron. It can also be regarded as connected networks between inputs
%at different time steps as shown in the right of Figure \ref{fig:rnn},
%so that information can be transported from the previous step to the
%next. Each neuron passes a message to a successor. The special
% framework of \textit{RNN} is particularly efficient for sequence input
% as in speech recognition and natural language processing. However,
% when the output is influenced by an input where there is a long time
% gap between them, it is unpredicted that \textit{RNN} neurons can
% still keep the related information.
Further as an extension,
\textit{LSTM} builds the long-term dependencies between the sequence
of outputs. The advantage of \textit{RNN} and \textit{LSTM} for sequence input provides
the same convenience for the continuous states of robotics.
%Several related applications are introduced in Section. \ref{sec:dsm}.

%YUN%%GAN
%\cite{goodfellow2014generative} proposed Genrative Adversarial Networks (\textit{GANs}) in recent years as an unsupervised method which trains a generator in an adversarial process with the discriminator. Specifically, the generator is trained to generate images from noise samples \emph{z} in order to fool the discriminator. Among the space of arbitrary functions, researchers wanted to find a unique solution, with generator recovering the training data distribution and discriminator equal to $\frac{1}{2}$ everywhere. Both generator and discriminator are with \textit{CNN} multilayer architecture and trained with backpropagation (Figure \ref{fig:gan} ). The objective of the \textit{GANs} is expressed as : $$\mathcal{L} = \mathbb{E}_{x\sim p_{data}(x)}[\mathrm{log}(D(x))] + \mathbb{E}_{x\sim p_z(z)}[\mathrm{log}(1-D(G(z)))]$$ where the generator $G$ is optimized to minimize the objective against the discriminator $D$ which to maximize it. \cite{goodfellow2014generative} pointed out the discriminator must be synchronized well with the generator during training, otherwise the generator will collapse too many values of noise \emph{z} to the same value of x to have enough diversity to model the data distribution.

%YUN%%GAN
%\begin{figure}[!ht]
%    \centering
%    \includegraphics[width=1\linewidth]{figs/gan2.pdf}
%    % \caption{Generator and Discriminator are trained simultaneously in an adversarial process. Both of them can be implemented by any form of differentiable function and trained with backpropagation. }
%    \caption{In Generative Adversarial Networks (GANs), the generator (G) and discriminator (D) are trained simultaneously in an adversarial process. Both of them can be implemented by any form of differentiable functions and trained with backpropagation. (z is the input noise vector of G)}
%    \label{fig:gan}
%\end{figure}

As for deep-learning models, these mentioned structures are
multi-layer nonlinear models and can be trained through gradient
descent methods. They can be used directly for feature
representations in supervised or unsupervised learning. For
reinforcement learning, it is more like an optimization problem. The
feature representation takes partial samples from the entire problem space. \citet
{mnih2013playing, mnih2015human} defined Deep Reinforcement Learning
(\textit{DRL}) by using a \textit{CNN} framework for feature
extractions through screen displays of Atari games. Not like the
ground-truth setting from a human in supervised learning, the agent in
\textit{DRL} is self-motivated through the interactions with the
environment based on the feedback scores. It surpassed the performance
of all previous algorithms and even accomplished a level comparable
with the best human player across a test set of 49 games. Various
problems in robotics can be considered as problems of reinforcement
learning naturally \citep{kober2013reinforcement}, so the success of
deep reinforcement learning motivates a lot of breakthroughs in
robotics which are introduced in Section \ref{sec:drlaaa}.

Deep-learning modules are often regarded as black boxes, which bring
lots of uncertainty. Actually, the convolutional filter is a
typical image processing method and \textit{CNN} can be regarded as a
deformation of the traditional mathematical model. For example,
Deformable Part Models (\textit{DPMs}) \citep{felzenszwalb2010cascade}
as graphical models (Markov Random fields), were once the state of art
in object detection task for RGB images.
\citet{girshick2015deformable} unrolled the \textit{DPM} algorithm and
represented each step in the \textit{DPM} to an identical \textit{CNN}
layer. Based on this synthesis, a learned feature extractor can
replace the hand-crafted feature like histograms of oriented gradients
(\textit{HOG}) and be connected with the \textit{DPM} directly.
\citet{zheng2015conditional} implemented Conditional Random Fields
(\textit{CRFs}) with Gaussian pairwise potentials as \textit{RNN},
which also combined the strengths of the probabilistic graphical model
and the deep-learning model. Because of the integration of these
models, both of the two projects made it possible to train the whole
deep network end-to-end. Finally, they dramatically improved the state
of art in object detection and semantics segmentation task in
conventional computer vision. In the regard of multi-level convolution,
the commonly used hand-crafted feature \textit{SIFT}
\citep{lowe1999object,lowe2004distinctive}, as a Gaussian Pyramid with
multi-scale convolutional filters can also be taken as a
\textit{CNN} model. We consider it is the essential reason why \textit{CNN}
can replace the effects of a similar generic hand-crafted feature, in applications such as place recognition.

For conventional robotics researchers, the review about
deep-learning \citep{lecun2015deep} (in aspects of data-mining or
image processing) written by Yann LeCun, Yoshua
Bengio, and Geoffrey Hinton is highly recommended for
further analysis and comparison.
%. The more
%experienced deep-learning researchers can directly choose the section
%of interest.
\subsection{Deep-learning in robotics: challenges} \label{sec:dlro}
\hl{this section is very important}

Deep-learning has shown great potential in artificial intelligence. As
a relative of artificial intelligence, robotics provides a fabulous
playground for deep-learning. However, robotics hold
several unique challenges for learning algorithms compared with other fields.

%uncertainty
\textbf{Uncertainty:} Robots do not always operate in controlled and
structured environment. Autonomous cars drive in outdoor environments
that may be crowded with pedestrians and vehicles; service robots run
in indoor environments that may contain variously appearances; industrial robots
may need to support a wide range of products; aerial robots can go across
low-altitude hybrid space, etc. Unlike the conventional distribution estimation in
data analysis (\textit{aka.} distributional uncertainty), significant uncertainty
may propagate unboundedly
in robotics applications in practical environments.
Although the assumptions of the noise model may solve partially a number
of practical problems, such as regular SLAM \citep{cadena2016past},
it is still difficult to solve a variety of practical problem with conventional methods.

Deep-learning is appropriate to solve, at least in part,
some of the problems with stronger uncertainty with the help from massive available data.
However, the success of
deep-learning is often attributed to the extremely high number of
parameters which is particularly useful for robotics. That is why
deep-learning is also criticized by serious over-fitting
to training samples. The dynamics in environments ask for a much higher capability to model robustness.
\citet{lenz2016deep} showed that over-fitting of deep-learning in
robotics can be reduced by carefully designed networks of the
deep-learning model, but there are still demanding research in this direction.

%evaluation metrics
\textbf{Evaluation Metrics}
For robots tasks, the output of the learning algorithms,
aims to make decisions, like whether the autonomous car should stop before a crossing street.
However, for conventional computer vision tasks, like classification and object detection,
the output is primarily a label prediction where the precision is highly emphasized regardless the predictive confidence.
But for robotics, the decision has to be checked carefully based on the confidence especially with series of prior and posterior when the human is in potentially hazardous conditions.
A single false output makes less sense for image classification,
but a false command can lead to disaster results in robotic practices.

\citet{grimmett2013knowing, grimmett2015introspective} proposed the
definition of introspection for robotics learning algorithms which is
also necessary for deep-learning methods. The classifier with high
introspection only makes mistakes with high uncertainty and output
correct result with high certainty, which is the definition of the
introspective quality of learning algorithms. Generally speaking,
because of the extreme uncertainty in robotics, traditional metrics
may be insufficient to characterize system performance of
deep-learning algorithms for robotics.

\textbf{Continuous States and Actions}
Note that besides the high-dimensional data and various uncertainty,
robotics are often connected with continuous actions and states and
the states of robotics are often non-deterministic. The general assumption like noise free and totally visible is impractical for
robotics. Because the cluster of small errors may lead to a totally different consequence, the maintenance of uncertainty is undoubtedly
necessary. As a partially observed system, sometimes true states
should be estimated by filters \citep{kober2013reinforcement}, e.g. such
problems are always critical in reinforcement learning procedures with
real robot platforms.

Another problem for learning in robotics is that it is often
unrealistic to implement the training procedure in the real world, such as that for reinforcement processes. The
trial-and-error process may lead to serious
damage to real systems. Most of the reinforcement learning
applications in robotics are trained in simulation environments
\citep{tai2015navigation,zhang2016vision}. However, model learned in
simulation alone unfortunately cannot be directly transferred to the real-world task.
With the development of deep-learning, this problem can be
partially solved by suitable initialization and post-tuning with real
world samples with transferred learning results\citep{tai2016towards}.

%
% \begin{table*}[ht!]
% \small
% \centering
% % \caption{The survey of deep-learning in robotic perceptions, based on the sensor used, model categorization, dataset source, real-time test, equal effect as a computer vision task, application, training efficiency and prediction precision.\label{tab:T1}}
% \caption{Categorization of robotic perception solutions using deep learning, based on the type of the on-board sensor, deep model, dataset source, real-world test, counterpart computer vision task, application, training efficiency and prediction precision.\label{tab:T1}}
% %￥\label{T:perception}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccccccc}
% \toprule
%
% % \multirow{2}{*}{Approach} & \multirow{2}{*}{Sensor} & Deep & Dataset&Real-time & \multirow{2}{*}{Effect} & \multirow{2}{*}{Application} &Training&\multirow{2}{*}{Precision}\\
% %  &   & Model & Source & Test& &&Efficiency&  \\
% \multirow{2}{*}{Approach} & \multirow{2}{*}{Sensor} & Deep & Dataset&Real-world & \multirow{2}{*}{Counterpart} & \multirow{2}{*}{Application} &Training&\multirow{2}{*}{Precision}\\
%  & & Model & Source & Test & Vision Task & & Efficiency &  \\
% \midrule
% \citet{lenz2015deep}  &  RGBD   & DNN  &   Benchmark
% & \checkmark &  Object Detection  & Grasping & $\bigstar \bigstar$ &$\bigstar$\\
% \midrule
% \citet{redmon2015real} & RGBD &  CNN &   Benchmark
% & \checkmark &  Object Detection  & Grasping& $\bigstar$ & $\bigstar \bigstar$\\
% \midrule
% \citet{livehicle}   &  3D Lidar & CNN  & Benchmark
% &     &Object Detection  & Auto Drive & $\bigstar$ & $ \bigstar$\\
% \midrule
% \citet{maturana2015conv3d}  & Lidar & 3D Conv &Self-Labeled& $\checkmark$ &Classification& Aerial &$\bigstar \bigstar$ &$\bigstar \bigstar$\\
% \midrule
% \citet{engelcke2016vote3deep}  & 3D Lidar & 3D Conv &Benchmark& $\checkmark$ &Object Detection& Auto Drive&$\bigstar \bigstar$ & $\bigstar \bigstar$\\
% \midrule
% \citet{yang2016realtime}  & RGB & CNN &Self-Labeled& $\checkmark$ &  Segmentation& SLAM &$\bigstar\bigstar\bigstar$ & $\bigstar\bigstar\bigstar$\\
% \midrule
% \citet{oliveira2016iros}  & RGB & CNN &Benchmark&  $\checkmark$ &Segmentation&Auto Drive &$\bigstar$ & $\bigstar\bigstar\bigstar$\\
% \midrule
% \citet{sunderhauf2015performance}  & RGB & CNN &Benchmark& $\checkmark$ &Classification&Auto Drive &$\bigstar$ & $\bigstar\bigstar$ \\
% \midrule
% \citet{sunderhauf2015place}  & RGB & CNN &Benchmark& $\checkmark$ &Object Detection& Auto Drive&$\bigstar\bigstar$ & $\bigstar\bigstar\bigstar$\\
%
% \bottomrule
% \end{tabular}}
% \end{table*}


==> secs/perception.tex <==
\hl{++++++++++++++++++++++++++++}
\section{Deep Learning for perception in robotics} \label{sec:percetpion}
\hl{============================}

Perception in robotics is quite similar to the conventional computer
vision tasks like image classification, object detection, and
semantics segmentation, where most of the models are trained with
supervised datasets as ground truth. In this section, perception
techniques for robotics fall into two categories: methods to extract
parts of the scene such as object detection, and those describe
the whole environment for place recognition. Generalized mobile robotics research also includes robot arms, so the related applications of deep learning in grasping and manipulation of robot arms were also surveyed. Several main related
publications in grasping, place recognition of autonomous driving and SLAM based on various metrics are listed in Table
\ref{tab:T1}.

\subsection{Object detection} \label{sec:dldetection}
The state-of-the-art object detection technique in computer vision is
based on region proposal algorithms by sharing convolutional features
with the detection network \citep{ren2015faster,redmon2015you} and
combined with the features from intermediate layers in \textit{CNN}
\citep{liu2015ssd}. The model, trained end-to-end, can output both the
bounding box and the class of the objects from the single image
directly. The same strategy was used for pedestrian detection for
autonomous cars \citep{angelova2015pedestrian, chen2016monocular,
angelova2015real}.
%YUN%% DCGAN
The unsupervised feature of \textit{GANs} can also be used to do tasks like classification and detection. \cite{radford2015unsupervised} applied the unsupervised representations to the classification of CIFAR-10 by vectorizing the representations of discriminator and added a regularized linear \textit{L2-SVM} classifier on top of them. After supervised training, the result outperforms K-means based approaches.

Besides RGB images, RGB-D data is also quite common nowadays and useful for robotics.
\citet{eitel2015multimodal} built a multi-modal learning framework by
taking both the RGB and depth image as input and processing them
separately for object recognition. Considering the fact that there is
always unpredicted noise in the real world, they proposed a depth
augmentation strategies, especially for robotics.
\citet{gupta2014learning} used \textit{CNN} to learn the features from
the geocentric encoding of the depth image, where object detection,
semantics segmentation and instance segmentation were output from the
model directly.
%YUN%% S2GAN
\cite{wang2016generative} considered an image as the production of structure and style. They proposed $S^2GAN$, which firstly generated a surface normal map and then mapped the texture onto the generated structure, to learn unsupervised RGB-D representations. They followed \textit{Fast-RCNN} method and modified the well-trained $S^2GAN$ to object detection tasks. The experiment showed potential result from the comparison with \textit{DCGAN} and \textit{AlexNet}.

Robot grasping is inherently a detection problem. Traditionally it was
solved through matching with full 3-D model
\citep{miller2004graspit,leon2010opengrasp,pelossof2004svm}, where a
strong prior information is necessary. \citet{jiang2011efficient} and
\citet{zhang2011grasp} converted that to a detection problem. It can then be solved through deep-learning methods with object
detection paradigm. As for robotic grasping in their work,
the goal is to derive the possible
location where the robot can execute grasping action through gripper.
Compared with conventional object detection problem, robust
performance and fast computation in grasp detection as part of the
control loop are extremely required so that the given object can
maximize the possibility of successful grasping efficiently. An
effective method in this field is required. Deep-learning
provides an effective solution.

Lenz \textit{et al.} successfully used a two-stage
\textit{DNN} to locate the grasp places through RGB-D information \citet{lenz2015deep}. A small-scale network was used to detect the potential and coarse grasp positions exhaustively and the other larger-scaled network was used to find the optimal graspable position. Note that the convolutional networks here were taken as a classifier in a sliding window detection pipeline, which was extremely time-consuming. Redmon \textit{et al.} trained the grasp detection end
to end through another convolutional networks \citet{redmon2015real}. Both of the detection accuracy and the computation speed were extremely improved. By integrating the bounding regression and object classification procedures, this model ran 150 times faster than previous methods. \citet{redmon2015real} also introduced a grid strategy as \textit{YOLO} \citep{redmon2015you} to propose multiple grasp positions in a single input. Further, \citet{johns2016deep} used \textit{CNN} to map the depth image to a grasp function by considering both the uncertainty of the grasp prediction and the location of the gripper.

Sparse point cloud captured from 3D Lidar like \textit{Velodyne} \footnote{http://velodynelidar.com} are widely applied in autonomous
vehicles. Such kind of information is quite similar to the depth image
from an RGB-D sensor, but with only sparse representation and mostly in an unorganized format.  Compared with RGB or RGB-D images, they provide a larger range of depth and are not influenced by lighting conditions. Deep-learning is also widely used for pedestrian and vehicle
detections in autonomous cars through sparse 3D points. \citet{livehicle} projected the 3D point cloud from \textit{Velodyne}
to a 2D point map and used a 2D convolutional network to achieve
vehicle detection. Conventional 2D convolutional layer was also
extended to 3D convolutional layer so that 3D point cloud can be
processed directly \citep{chen2016multiview,li20163dfully,wang2015voting,engelcke2016vote3deep,maturana2015voxnet}.
Amongst, \citet{chen2016deeplab} used a combined network of taking
the bird view and the front view of the Lidar and the RGB
image all together as the input. \citet{engelcke2016vote3deep}
combined voting in sparse point cloud with 3D convolutional sliding
window and saved a lot of useless calculation in sparse area.
\citet{maturana2015conv3d} applied 3D convolutional neural networks to detect the landing zone for aerial robots.

Based on the success of Fully Convolutional Networks (\textit{FCN})
\citep{long2015fully} on semantics segmentation,
\citet{yang2016realtime} built a \textit{CNN} model to extract the
ground and wall planes from a single image. Based on these plane
features extracted by the deep-learning method, a SLAM framework
\citep{yangpop} was also implemented. \citet{oliveira2016iros} used
the same strategy for the road segmentation and lane prediction
applied on the autonomous vehicles.
%YUN%% SALGAN
%Visual saliency prediction can help extract ROIs from images and further reduce the input dimension of visual tasks. For instance, visual saliency predictions of drivers could help improve the accuracy and real-time performance of autonomous driving techniques.
\cite{pan2017salgan} explored adversarial training to visual saliency prediction. Instead of unsupervised training, the inputs are images and their corresponding saliency maps. They compared different metrics with/without adversarial training and concluded that adversarial training improves the saliency prediction result in most of the metrics.

The success of \textit{RNN} in object tracking
\citep{ondruska2016deep} was also leveraged for autonomous driving.
\citet{dequaire2016deep} predicted future states of the objects based
on the current inputs through a \textit{RNN} model.

Some rarely used sensor information is also considered as the input
for deep-learning model. Through tactile sensor on the end effector,
object and material detection were also implemented through
deep-learning \citep{schmitz2014tactile, shiv2016robust}.
\citet{valada15isrr} achieved terrain classification through the
acoustic sensor mounted at the bottom of vehicles.

%YUN%% Anomalies detection
%Some researchers applied \textit{GANs} in anomalies detections. It could be traced back to \cite{schlegl2017unsupervised}, where researchers started to detect anomalies in medical images with \textit{GANs}. \cite{lawson2017finding} applied \textit{GANs} on mobile robots for a patrol task and demonstrated that the latent space features could be used to locate anomalies in indoor environments.

\subsection{Place recognition} \label{sec:dlplace}

Visual place recognition is an extremely challenging problem considering the variety weather conditions, time-of-day, and environmental dynamics. Given an
image of a place, mobile robots are requested to recognize
a previously seen place \citep{lowry2016visual}.
With the development of autonomous cars, such kind of recognition is
strongly demanding. The difficulties to realize robust place
recognition include the perceptual aliasing (similar places), various
viewpoints and other appearance variation during the revisits.

Trained in the dataset with millions of labeled images like
\textit{Imagent} \citep{deng2009imagenet}, the state-of-art
\textit{CNN} model showed great generalities in different vision tasks
including scene understanding
\citep{Razavian2014CVPR,donahue2014decaf}. Even with simple linear
classifiers, \textit{CNN} features outperformed sophisticated
kernel-based methods with hand-crafted features
\citep{donahue2014decaf}. And it can quickly be transformed to other
tasks with rarely labeled samples as references
\citep{Razavian2014CVPR}. Even for the task like camera
re-localization with extremely serious demand for place recognition
precision, convolutional features also showed huge improvement
compared with \textit{SIFT}-based localizes
\citep{kendall2015posenet}. Application in place recognition for
mobile robots were naturally motivated
\citep{chen2014convolutional,sunderhauf2015performance}.

\citet{sunderhauf2015performance} tested the performance of several
popular convolutional networks models for the global feature
abstraction of place recognition. It showed that networks trained for
semantic place categorization
\citep{zhou2014learning,liao2016understand} were more effective than
those trained for object detection \citep{girshick2014rich}. The
utility of convolutional features for visual place recognition in
robotics was proved as well. It also proposed that mid and high-level
features from the \textit{CNN} models were more robust for the changes
of appearance and viewpoint. \citet{naseer2015robust} and
\citet{arroyo2016fusion} showed that features extracted by
convolutional models for place recognition were evidently stable
for extreme changes across the fours seasons.

%motivated by some work
\citet{sunderhauf2015place} proposed a pipeline similar to object
detection but for visual place recognition. \textit{CNN}
models were adopted to recognize the landmarks which are located by Edge
Boxes, and an object proposal method \citep{zitnick2014edge} was used as
traditional object detection. Based on the similar place objects
(buildings, squares, \textit{etc.}), conventional object proposals and
recognition were stable enough over significant viewpoints and
condition changes, which make it suitable for place
recognition.

\citet{arandjelovic2015netvlad} combined the features extracted from
\textit{CNN} models with Vector of Locally Aggregated Descriptors
(\textit{VLAD}) \citep{jegou2010aggregating}. They built an end-to-end
model for place recognition task compared with the former methods
where \textit{CNN} was only used for feature recognition
\citep{chen2014convolutional}. The end-to-end training motivated the
model to be trained life-long time with the continuously collected
images from Google Street View. The recognition precision for places
on benchmark datasets was improved a lot.

%YUN%%IROS2017ADA
In order to deal with the big appearance change in place recognition, some researchers adopt \textit{GANs} to generate a fake representation from the original input to eliminate appearance change. \cite{latif2017addressing} trained a coupled \textit{GAN} to achieve this goal. Their network architecture is similar to \cite{zhu2017unpaired} which is with cyclic constraints to enforce a bijection of two domain, and trained with unpaired datasets in two different domain. Their experiment showed that the discriminator features have small cosine distance if the input images are close in appearance. This means that the features robust to appearance changes can be derived from \textit{GANs} which act as the domain adaptor of two domains. \cite{wulfmeier2017addressing} solved this problem with adversarial domain adaptation method to maximize the performance of a supervised task both in the source domain and target domain. They proposed a method to adapt supervised network directly to align the features of two domains. They further extended this work into semantic segmentation and demonstrated that the aligned features could also be used in free-space segmentation task.

The success of \textit{CNN} features on place recognition of robots
reciprocally provide much more possibility for interesting ideas, like
matching the ground-level image with a database collected from aerial
robots \citep{lin2015learning} and using 2D occupancy grids
constructed by Lidar to classify the place categorization (into a corridor,
doorway, room, etc.) \citep{goeddel2016learning}.

\subsection{Scene understanding}


\subsection{Future directions}
\subsubsection{Multimodal}
There are various sensors adapted for robotics. Right now, the
\textit{DL}-related applications are mainly about extracting
features from images, following the trend of deep-learning in computer
vision. Multi-modal combination by taking different raw sensor
information (RGB, RGB-D, Lidar, \textit{etc.}) as input
\citep{eitel2015multimodal} is still deserved to explore.
\citet{liao2016parse} predicted the depth of the image by taking the
raw image and a single-line 2D-lidar reflection as input, which showed
that \textit{CNN} models can help to find the essential relations
between different sensor information. Further study is necessary
to enhance the robustness of output.
\subsubsection{3D Convolution}
Autonomous driving is one of the most popular topics in both robotics
and artificial intelligence. As we mentioned in Section
\ref{sec:dldetection}, there have been some pedestrians and vehicles
detection tasks through the widely used 3D Lidar on autonomous vehicles.
However, up-to-date 3D convolution processes are simply
extending the 2D convolutional filters to a 3D version.
\citet{wang2015voting} and \citet{engelcke2016vote3deep} explored that
voting could be regarded as a convolution process and built a combined
model by taking voting as a layer of 3D convolution. We believe such
kind of effective combinations between the deep-learning and
traditional approaches will bring further breakthroughs in perception.
\subsubsection{Pix-level place recognition}
In Section \ref{sec:dlplace}, most introduced methods are based on
global \textit{CNN} features, and object detection pipelines were
proposed to solve the place recognition problem. Besides that, semantic
segmentation methods \citep{zheng2015conditional,long2015fully} can
provide more precise features. The related high-level representations
of the places can overcome the challenges for various appearance and viewpoints
in the same scene.
%YUN%%Metric
%\subsubsection{Metric}
%Since \textit{GANs} were firstly proposed by Goodfellow et.al, multiple variants of \textit{GANs} followed it from unsupervised learning to supervised learning. Even though each paper claimed that their \textit{GANs} were able to generate images with higher resolution and fewer artifacts, they just made the qualitative comparison with human intuition or by transforming the learned representation to traditional visual tasks. In this way, the model might perform well in specific tasks, but we are still not aware of the general effectiveness of each model. Recently, \cite{mario2017are} provided a comparison of multiple variants of \textit{GANs} with Fr´echet Inception Distance (FID), which is a quantitative metric proposed by \cite{heusel2017gans}, and claimed that the tested \textit{GANs} variants reached similar values of FID. % Need to further explore

\subsubsection{End-to-end}
An essential reason to perform \textit{DL} with hierarchical
convolutional operations
\citep{girshick2015deformable,zheng2015conditional,engelcke2016vote3deep}
is to build the end-to-end model. The end-to-end model trained through
back-propagation dramatically speed up the time for calculation
\citep{arandjelovic2015netvlad}. Compared with pure feature
extractions such as that in \citep{Razavian2014CVPR}, end-to-end model brings a lot of
efficiency and convenience. End-to-end solutions, aka model-less methods, to robotic problems
are also promising for complex tasks.

% control for obstacle avoidance
%environment recognition for classification \cite{tai2016deep}
%Giusti \cite{giustimachine} use a deep-learning framework to perceive a forest trail for a quadrotor. The target is to output a related moving direction taking a single RGB image as input. Because of the huge variability of the appearance, this task is quite difficult. The deep neural network even performs better than the human decision in unseen place test.

